Discovery of the missing intermediate-mass helium stars stripped in binaries

The theory of binary evolution predicts that many massive stars should lose their hydrogen-rich envelopes via interaction with a companion -- revealing hot helium stars with masses of $\sim$2--8M$_{\odot}$. However, only one candidate system had been identified, leaving a large discrepancy between theory and observation. Here, we present a new sample of stars -- identified via excess ultraviolet emission -- whose luminosities, colors, and spectral morphologies are consistent with predictions for the missing population. We detect radial velocity variations indicative of binary motion and measure high temperatures ($T_{\rm eff}\sim60-100$kK), high surface gravities ($\log(g)\sim5$) and depleted surface hydrogen mass fractions ($X_{\rm{H,surf}}\lesssim0.3$), which match expectations for stars with initial masses between 8--25 M$_{\odot}$ that have been stripped via binary interaction. These systems fill the helium star mass gap between subdwarfs and Wolf-Rayet stars, and are thought to be of large astrophysical significance as ionizing sources, progenitors of stripped-envelope supernovae and merging double neutron stars.

==> Tables/table_mdot_EW.tex <==
\begin{tabular}{lcccccc}\\ 
\toprule \midrule 
$\dot{M}_{\mathrm{wind}}$ [$M_{\odot}$/yr] & He\textsc{ii} $\lambda$3835+H$\eta$ & He\textsc{i}+\textsc{ii} $\lambda$4026 & He\textsc{ii} $\lambda$4100+H$\delta$ & He\textsc{ii} $\lambda$4860+H$\beta$ & He\textsc{ii} $\lambda$5411 & He\textsc{i} $\lambda$5876\\ 
\midrule 
$10^{-7}$ & 0.29 & 0.69 & 1.74 & 2.16 & 2.04 & 0.08\\ 
$3\times10^{-8}$ & 0.31 & 0.70 & 1.88 & 2.54 & 2.15 & 0.10\\ 
$10^{-8}$ & 0.31 & 0.70 & 1.90 & 2.53 & 1.99 & 0.12\\ 
$3\times10^{-9}$ & 0.32 & 0.72 & 1.92 & 2.53 & 1.96 & 0.12\\ 
$10^{-9}$ & 0.32 & 0.71 & 1.92 & 2.53 & 1.94 & 0.12\\ 
\bottomrule
\end{tabular}
